Closing the Gap -- Formally Verifying Dynamically Typed Programs like Statically Typed Ones Using Hoare Logic -- Extended Version --

Dynamically typed object-oriented languages enable programmers to write elegant, reusable and extensible programs. However, with the current methodology for program verification, the absence of static type information creates significant overhead. Our proposal is two-fold: First, we propose a layer of abstraction hiding the complexity of dynamic typing when provided with sufficient type information. Since this essentially creates the illusion of verifying a statically-typed program, the effort required is equivalent to the statically-typed case. Second, we show how the required type information can be efficiently derived for all type-safe programs by integrating a type inference algorithm into Hoare logic, yielding a semi-automatic procedure allowing the user to focus on those typing problems really requiring his attention. While applying type inference to dynamically typed programs is a well-established method by now, our approach complements conventional soft typing systems by offering formal proof as a third option besides modifying the program (static typing) and accepting the presence of runtime type errors (dynamic typing).

==> Makefile <==
# since they aren't file names
.phony: all clean

all: images
# figures
	pdflatex ${NAME} && bibtex ${NAME} && pdflatex ${NAME} && pdflatex ${NAME}
#	ghc --make TeXFigures.hs -main-is TeXFigures.main -o TeXFigures && \
	./TeXFigures && \

IMGSRCS=$(wildcard images/*.pdf_tex)
IMGS=$(IMGSRCS:.pdf_tex=.tex)

images: $(IMGS)

.SUFFIXES: .pdf_tex

.pdf_tex.tex: $(IMGS)
	perl -ne 's/(\[width=\\unitlength\]\{)/\1images\//g;print' $< > $@

clean:
	rm *~ core ${NAME}.bbl ${NAME}.aux ${NAME}.blg ${NAME}.log ${NAME}.toc texput.log
# images/*.tex also, presumably

package: archiv.tar.gz
        mkdir archiv;
        cp -r * archiv/;
        tar -cvvf archiv.tar archiv/;
        gzip archiv.tar


==> appendices/app_type_hoare_logic.tex <==
\todo{the algorithm is now flow-sensitive! Adapt rules accordingly!}

\vspace{0.1cm}
\noindent AXIOM: $\restricted$-CONST
%
\begin{center}
$\{\tau\} \Vnull \{\tau \wedge \llbracket \result \rrbracket \in \{\}\}$
\end{center}\todo{would null be permitted within brackets, this would be same as HL. neccessary?}

\noindent AXIOM: $\restricted$-VAR
%
\begin{center}
$\{\tau[\result := \PL{u}]\} \PL{u} \{\tau\}$ \hspace{1cm} where $\PL{u} \in \Var_L$.
\end{center}\todo{same as HL. neccessary?}
%

\noindent AXIOM: $\restricted$-IVAR

\begin{center}
$\{p\} @v \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$
\end{center}

where $p \rightarrow \llbracket \this.@v \rrbracket \in \BaseTypeX$, $\BaseTypeX \in 2^{\Class}$, $@v \in \Var_I$.


\noindent RULE: $\restricted$-ASGN - FLOW INSENSITIVE %(both normal and instance variables)
\begin{center}
\AxiomC{$\{p\} E \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$}
\RightLabel{with $v \in \Var_L$}
\UnaryInfC{$\{p\} v := E \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$}
\DisplayProof
\end{center}
%
where $p \equiv p' \wedge \llbracket v \rrbracket \in \BaseTypeX'$,
$v \not\in \free(p'), \BaseTypeX, \BaseTypeX' \in 2^{\Class}, \BaseTypeX \subseteq \BaseTypeX'$.

\noindent RULE: $\restricted$-IASGN - FLOW INSENSITIVE %(both normal and instance variables)
\begin{center}
\AxiomC{$\{p\} E \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$}
\RightLabel{with $@v \in \Var_I$}
\UnaryInfC{$\{p\} @v := E \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$}
\DisplayProof
\end{center}
%
where $p \equiv \TInv \wedge p'$,
$p' \rightarrow \llbracket this \rrbracket \in \{C\}$,
$@v \not\in \free(p'), \BaseTypeX \in 2^{\Class}$, $\BaseTypeX \subseteq \BaseTypeX_{C.@v}$.

\todo{use $\sqsubseteq$ instead of $\subseteq$ for types!!!}

\noindent RULE: $\restricted$-SEQ

\begin{center}
\AxiomC{$\{p\} S_1 \{r \wedge \llbracket \result \rrbracket \in \BaseTypeX_1\}$}
\AxiomC{$\{r\} S_2 \{q\}$}
\BinaryInfC{$\{p\} S_1; S_2 \{q\}$}
\DisplayProof
\end{center}

with $\BaseTypeX_1 \in 2^{\Class}$

\noindent RULE: $\restricted$-COND - PATH INSENSITIVE %(strong typesafe partial correctness)
%
% \begin{center}
% \AxiomC{$\begin{matrix}
%           \{p \wedge bool(B,true)\} S_1 \{q \wedge \llbracket result \rrbracket = T_1\} \\
%           \{p \wedge bool(B,false)\} S_2 \{q \wedge \llbracket result \rrbracket = T_2\}
%          \end{matrix}$}
%        
% \UnaryInfC{$\{p \wedge bool(B)\}$ if $B$ then $S_1$ else $S_2$ fi $\{q \wedge \llbracket result \rrbracket = T_1 \sqcup T_2\}$}
% \DisplayProof
% \end{center}
%
\begin{center}
\AxiomC{$\begin{matrix}
          \{p\} B \{p \wedge \llbracket \result \rrbracket \in \{bool\}\} \\
          \{p\} S_1 \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX_1\} \\
          \{p\} S_2 \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX_2\}
         \end{matrix}$}
       
\UnaryInfC{$\{p\}$ if $B$ then $S_1$ else $S_2$ fi $\{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$}
\DisplayProof
\end{center}
%
where $\BaseTypeX_1 \subseteq \BaseTypeX, \BaseTypeX_2 \subseteq \BaseTypeX, \BaseTypeX,\BaseTypeX_1,\BaseTypeX_2 \in 2^{\Class}$.

\noindent RULE: $\restricted$-LOOP
\begin{center}
\AxiomC{$\begin{matrix}
          \{p\} B \{p \wedge \llbracket \result \rrbracket \in \{bool\} \} \\
          \{p\} S \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}
         \end{matrix}$}
\UnaryInfC{$\{p\}$ while $B$ do $S$ od $\{p \wedge \llbracket \result \rrbracket \in \{\}\}$}
\DisplayProof
\end{center}

where $\BaseTypeX \in 2^{\Class}$.

\noindent RULE: $\restricted$-BLCK
%
\begin{center}
\AxiomC{$\{p\} S \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$}
%\RightLabel{ where $\result \not\in \{\Vector{x}\}$}
\UnaryInfC{$\{p'\}$ begin local $\Vector{u} := \Vector{t}; S \text{ end} \{\TInv \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$}
\DisplayProof
\end{center}
%
where $p' \rightarrow p[\Vector{u}\Vector{\overline{u}} := \Vector{t}\Vector{\PL{null}}]$, $\{\Vector{u}\} \subseteq \Var_L \setminus \{\result\}$ and $\{\Vector{t}\} \subseteq \Var_L \cup \{\PL{null}\}$.

% \noindent RULE: $\restricted$-PASGN
% 
% \begin{center}
% $\{p[x_1,...,x_n := t_1,...,t_n] \wedge \llbracket t_n \rrbracket \in \BaseTypeX\} x_1,...,x_n := t_1,...,t_n \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$
% \end{center}

\noindent RULE: $\restricted$-METH
%
\begin{center}
\AxiomC{$\begin{matrix}
          \{p\} E_i \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX_i \} \text{ for } i \in \mathbb{N}_n \\
          \{p_j\} l_0.m(l_1,...,l_n) \{\TInv \wedge \llbracket \result \rrbracket \in \BaseTypeX'_j\} \text{ for } j \in \mathbb{N}^1_k
         \end{matrix}$}
       
\UnaryInfC{$\{p\} E_0.m(E_1,...,E_n) \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$}
\DisplayProof
\end{center}
%
\todo{these are union types, not basetypes!!! (do not use $\BaseTypeX$, but $\UnionTypeX$)}
%
where $\BaseTypeX_0 = \{C_1,...,C_k\}$,
$p_j \equiv \TInv \wedge \llbracket l_0 \rrbracket \in \{C_j\} \wedge \bigwedge\limits_{i = 1}^n \llbracket l_i \rrbracket \in \BaseTypeX_{ij}$,
$p \wedge \llbracket l_0 \rrbracket \in \{C_j\} \rightarrow p_j$,
$\BaseTypeX'_j \subseteq \BaseTypeX$ and $\BaseTypeX_i \subseteq \BaseTypeX_{ij}$ for $i \in \mathbb{N}^1_n, j \in \mathbb{N}^1_k$.

\noindent RULE: $\restricted$-REC
%
\begin{center}
\AxiomC{$\begin{matrix}
          A \vdash \{p\} S \{q\}, \\
          A \vdash \{p_i\} \text{begin local }\this, \Vector{u_i} := l_i,\Vector{v_i}; S_i \text{ end} \{q_i\}, i \in \mathbb{N}^1_n \\
          p_i \rightarrow \llbracket l_i \rrbracket \in \{C_i\}, i \in \mathbb{N}^1_n
         \end{matrix}$}
       
\UnaryInfC{$\{p\} S \{q\}$}
\DisplayProof
\end{center}
%
where method $m_i(\Vector{u_i}) \{ S_i \} \in \Method_{C_i}$ for $i \in \mathbb{N}^1_n$ and $A \equiv \{p_1\} l_1.m_1(\Vector{v_1}) \{q_1\}, ..., \{p_n\} l_n.m_n(\Vector{v_n}) \{q_n\}$.


\noindent AXIOM: $\restricted$-NEW
\begin{center}
$\{p\} \mathbf{new}_C \{p \wedge \llbracket \result \rrbracket \in \{C\}\}$
\end{center}


\subsection{Soundness}

The rules given can be composed from the rules for typesafe partial correctness of \textbf{dyn} programs.

%\noindent :
\begin{proof}[RULE $\restricted$-ASGN]\hspace{0.1cm}\newline
 \begin{center}
  \AxiomC{$\{p\} E \{ p \wedge \llbracket \result \rrbracket \in \BaseTypeX \}$}
  \RightLabel{\scriptsize(CONS)}
  \UnaryInfC{$\{p\} E \{ p' \wedge \llbracket \result \rrbracket \in \BaseTypeX' \wedge \llbracket \result \rrbracket \in \BaseTypeX \}$}
  \RightLabel{\scriptsize(ASGN)}
  \UnaryInfC{$\{p\} v := E \{ p' \wedge \llbracket v \rrbracket \in \BaseTypeX' \wedge \llbracket \result \rrbracket \in \BaseTypeX \}$}
  \RightLabel{\scriptsize(CONS)}
  \UnaryInfC{$\{p\} v := E \{ p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$}
  \DisplayProof
 \end{center}
 with $\BaseTypeX \subseteq \BaseTypeX'$, $p \equiv p' \wedge \llbracket v \rrbracket \in \BaseTypeX'$, $v \not\in \free(p')$
 \hfill$\Box$
\end{proof}

\begin{proof}[RULE $\restricted$-IASGN]\hspace{0.1cm}\newline
 \begin{center}
  \AxiomC{$\{p\} E \{ p \wedge \llbracket \result \rrbracket \in \BaseTypeX \}$}
  \RightLabel{\scriptsize(CONS)}
  \UnaryInfC{$\{p\} E \{ \TInv[this.@v := \result] \wedge p' \wedge \llbracket \result \rrbracket \in \BaseTypeX \}$}
  \RightLabel{\scriptsize(ASGN)}
  \UnaryInfC{$\{p\} @v := E \{ \TInv \wedge p' \wedge \llbracket \result \rrbracket \in \BaseTypeX \}$}
  \RightLabel{\scriptsize(CONS)}
  \UnaryInfC{$\{p\} @v := E \{ p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$}
  \DisplayProof
 \end{center}
 with $\BaseTypeX \subseteq \BaseTypeX_{C.@v}$, $p \equiv \TInv \wedge p'$, $@v \not\in \free(p')$, $p' \rightarrow \llbracket this \rrbracket \in \{C\}$, $p \rightarrow \llbracket this.@v \rrbracket \in \BaseTypeX_{C.@v}$.

 the upper application of the CONS-rule needs further explanation:
 $\TInv$ can we written as a universally quantified conjunction of statements of the following form
 \[ \llbracket o \rrbracket \in \{C'\} \rightarrow \llbracket o.@u \rrbracket \in \BaseTypeX_{C'.@u} \]
 Now we consider an application of the substitution $[this.@v := \result]$ to the above statement:
 Since assignments to $@\mathbf{c}$ are not allowed in programs, we can safely assume that $@v \not= @\mathbf{c}$
 and conclude $\llbracket o \rrbracket \in \{C'\}[this.@v := \result] \equiv \llbracket o \rrbracket \in \{C'\}$.
 The left-hand side of the implication is thus unaffected by the substitution. For the right-hand side we
 have to distinguish the following cases
\begin{itemize}
 \item $@u \not= @v$:
 \[ \llbracket o.@u \rrbracket \in \BaseTypeX_{C'.@u}[this.@v := \result] \equiv \llbracket o.@u \rrbracket \in \BaseTypeX_{C'.@u} \]
 \item $@u = @v$:
 \begin{align*}
  \llbracket o.@u \rrbracket & \in \BaseTypeX_{C'.@u}[this.@v := \result] \equiv \\
  & \text{if } o = this \text{ then } \llbracket \result \rrbracket \in \BaseTypeX_{C'.@v} \text{ else } \llbracket o.@u \rrbracket \in \BaseTypeX_{C'.@u} \text{ fi}
 \end{align*}
\end{itemize}
From the first case, we see that all cases with other instance variables than the one assigned to are
also unaffected by the substitution.
Furthermore, $\llbracket this \rrbracket \in \{C\}$ and $\llbracket o \rrbracket \in \{C'\}$ with
$C \not= C'$ imply $o \not= this$. Hence, for all cases where the type of $o$ does not coincide with the type
of $this$, the above conditional is equivalent to its false branch $\llbracket o.@u \rrbracket \in \BaseTypeX_{C'.@u}$ and
the statement is thus unaffected by the substitution.
Summarizing, the substitution introduces a conditional in exactly one case: the one dealing with
the instance variable $@v$ of class $C$. For this case, we substitute the conditional by an equivalent
logical formula and get
\begin{align*}
 \llbracket o \rrbracket \in \{C\} \rightarrow & o \not= this \rightarrow \llbracket o.@v \rrbracket \in \BaseTypeX_{C.@v} \wedge \\
 \llbracket o \rrbracket \in \{C\} \rightarrow & o = this \rightarrow \llbracket \result \rrbracket \in \BaseTypeX_{C.@v}.
\end{align*}
%
Since $o = this$ implies $\llbracket o \rrbracket \in \{C\}$, we can write the entire substitution as follows
\[ \TInv[this.@v := \result] \leftrightarrow \TInv' \wedge \forall o \quantsep o = this \rightarrow \llbracket \result \rrbracket \in \BaseTypeX_{C.@v} \]
%
where $\TInv'$ is equivalent to $\TInv$ except for an added $o \not= this \rightarrow$ in the case for $C.@v$.
In fact, we can further simplify this to
%
\[ \TInv[this.@v := \result] \leftrightarrow \TInv' \wedge \llbracket \result \rrbracket \in \BaseTypeX_{C.@v}. \]

and since $\TInv \rightarrow \TInv'$ and $\BaseTypeX \subseteq \BaseTypeX_{C.@v}$, we have $p \wedge \llbracket \result \rrbracket \in \BaseTypeX \rightarrow \TInv[this.@v := \result]$.
 \hfill$\Box$
\end{proof}

\todo{$\restricted$-NEW rule}

% TODO{proof COND rule}
% \noindent RULE $\restricted$-COND:
% 
% \begin{center}
% \AxiomC{$\begin{matrix}
%           \{p\} B \{p \wedge \llbracket \result \rrbracket \in \{bool\}\} \\
%           \{p\} S_1 \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX_1\} \\
%           \{p\} S_2 \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX_2\}
%          \end{matrix}$}
% \RightLabel{\scriptsize(2x CONS,)}
% \UnaryInfC{$\begin{matrix}
%           \{p\} B \{p \wedge \mathit{bool\_test} \} \\
%           \{p \wedge b\} S_1 \{q\} \\
%           \{p \wedge \neg b\} S_2 \{q\}
%          \end{matrix}$}
% \RightLabel{\scriptsize(COND)}
% \UnaryInfC{$\{p\}$ if $B$ then $S_1$ else $S_2$ fi $\{q\}$}
% \RightLabel{\scriptsize(CONS)}
% \UnaryInfC{$\{p\}$ if $B$ then $S_1$ else $S_2$ fi $\{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$}
% \DisplayProof
% \end{center}
% where $\BaseTypeX_1 \subseteq \BaseTypeX, \BaseTypeX_2 \subseteq \BaseTypeX, \BaseTypeX,\BaseTypeX_1,\BaseTypeX_2 \in 2^{\Class}$.
% 
% where $q \equiv p \wedge \llbracket \result \rrbracket \in \BaseTypeX_1 \vee \llbracket \result \rrbracket \in \BaseTypeX_2$
% 
% %TODO{update proof ($\BaseTypeX_1$ and $\BaseTypeX_2$)}
% 
% \begin{proof}
%  One takes the CONDITIONAL Rule for typesafe partial correctness (in which $bool(\result,b) \leftrightarrow \llbracket \result \rrbracket \in \{bool\}$),
%  sets $r \equiv p$ and $q \equiv p \wedge \llbracket x_1 \rrbracket \in \BaseTypeX \wedge \llbracket x_2 \rrbracket \in \BaseTypeX$
%  and adds an application of the CONSEQUENCE Rule afterwards ($[p \wedge g \leftrightarrow wlp(b,B)] \rightarrow p$
%  and $p \wedge \llbracket x_1 \rrbracket \in \BaseTypeX \wedge \llbracket x_2 \rrbracket \in \BaseTypeX \wedge \result = $ if $g$ then $x_1$ else $x_2$ fi $\rightarrow p \wedge \llbracket \result \rrbracket \in \BaseTypeX$).
%  \BaseTypeXhen, the proposition $\{p \wedge b\} S_1 \{p \wedge \llbracket x_1 \rrbracket \in \BaseTypeX \wedge \llbracket x_2 \rrbracket \in \BaseTypeX \wedge \result = x_1\}$ can be derived
%  by applying the CONSEQUENCE Rule before the CONDITIONAL rule ($p \wedge b \rightarrow p$ and $p \wedge \llbracket \result \rrbracket \in \BaseTypeX \rightarrow [p \wedge \llbracket x_1 \rrbracket \in \BaseTypeX \wedge \llbracket x_2 \rrbracket \in \BaseTypeX \wedge \result = x_1 ]$)
%  %TODO{last sentence is wrong -> fix this proof!}
% \end{proof}

% updates rules:
% \noindent RULE: $\restricted$-BLCK
% %
% \begin{center}
% \AxiomC{$\{p\} S \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$}
% %\RightLabel{ where $\result \not\in \{\Vector{x}\}$}
% \UnaryInfC{$\{p'\}$ begin local $\Vector{u} := \Vector{t}; S \text{ end} \{\llbracket \result \rrbracket \in \BaseTypeX\}$}
% \DisplayProof
% \end{center}
% %
% where $p' \rightarrow p[\Vector{u}\Vector{\overline{u}} := \Vector{t}\Vector{\PL{null}}]$, $\{\Vector{u}\} \subseteq \Var_L \setminus \{\result\}$ and $\{\Vector{t}\} \subseteq \Var_L \cup \{\PL{null}\}$.
% 
% % \noindent RULE: $\restricted$-PASGN
% % 
% % \begin{center}
% % $\{p[x_1,...,x_n := t_1,...,t_n] \wedge \llbracket t_n \rrbracket \in \BaseTypeX\} x_1,...,x_n := t_1,...,t_n \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$
% % \end{center}
% 
% \noindent RULE: $\restricted$-METH
% %
% \begin{center}
% \AxiomC{$\begin{matrix}
%           \{p\} E_i \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX_i \} \text{ for } i \in \mathbb{N}_n \\
%           \{p_j\} l_0.m(l_1,...,l_n) \{\TInv \wedge \llbracket \result \rrbracket \in \BaseTypeX'_j\} \text{ for } j \in \mathbb{N}^1_k
%          \end{matrix}$}
%        
% \UnaryInfC{$\{p\} E_0.m(E_1,...,E_n) \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$}
% \DisplayProof
% \end{center}
% %
% where $\BaseTypeX_0 = \{C_1,...,C_k\}$,
% $p_j \equiv \TInv \wedge \llbracket l_0 \rrbracket \in \{C_j\} \wedge \bigwedge\limits_{i = 1}^n \llbracket l_i \rrbracket \in \BaseTypeX_{ij}$,
% $p \wedge \llbracket l_0 \rrbracket \in \{C_j\} \rightarrow p_j$,
% $\BaseTypeX'_j \subseteq \BaseTypeX$ and $\BaseTypeX_i \subseteq \BaseTypeX_{ij}$ for $i \in \mathbb{N}^1_n, j \in \mathbb{N}^1_k$.
% 
% \noindent RULE: $\restricted$-REC
% %
% \begin{center}
% \AxiomC{$\begin{matrix}
%           A \vdash \{p\} S \{q\}, \\
%           A \vdash \{p_i\} \text{begin local }\this, \Vector{u_i} := l_i,\Vector{v_i}; S_i \text{ end} \{q_i\}, i \in \mathbb{N}^1_n \\
%           p_i \rightarrow \llbracket l_i \rrbracket \in \{C_i\}, i \in \mathbb{N}^1_n
%          \end{matrix}$}
%        
% \UnaryInfC{$\{p\} S \{q\}$}
% \DisplayProof
% \end{center}
% %
% where method $m_i(\Vector{u_i}) \{ S_i \} \in \Method_{C_i}$ for $i \in \mathbb{N}^1_n$ and $A \equiv \{p_1\} l_1.m_1(\Vector{v_1}) \{q_1\}, ..., \{p_n\} l_n.m_n(\Vector{v_n}) \{q_n\}$.



\begin{proof}[RULE: $\restricted$-METH]\hspace{0.1cm}\newline
 \todo{incorporate usage of $TInv$ to derive types for instance variables of the calee into this rule}
 \todo{proof again from HL with quantification over objects and object creation}
\begin{center}
% \AxiomC{$\begin{matrix}
%           \{p\} E_i \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX_i \} \text{ for } i \in \mathbb{N}_n \\
%           \{p_j\} l.m(l_1,...,l_n) \{p_j \wedge \llbracket \result \rrbracket \in \BaseTypeX'_j\} \text{ for } j \in \mathbb{N}^1_k
%          \end{matrix}$}
       
\AxiomC{$\begin{matrix}
          \{p_i\} E_i \{p_{i+1}[l_i := \result] \} \text{ for } i \in \mathbb{N}_n & (1)\\
          \{p_{n+1}\} l_0.m(l_1,...,l_n) \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\} & (2)
         \end{matrix}$}
\RightLabel{\scriptsize(METH)}
\UnaryInfC{$\{p\} E_0.m(E_1,...,E_n) \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$}
\DisplayProof
\end{center}
%

where $p_i \equiv p \wedge \bigwedge\limits_{j = 0}^{i-1} \llbracket l_j \rrbracket \in \BaseTypeX_j$, $l_i \in \Var, l_i \not\in free(E_j) \cup change(E_j)$ for all $i,j \in \mathbb{N}_n$.

Using the fact that the $l_i$ are not modified by the $E_j$, $(1)$ can be derived from the premises of $\restricted$-METH by
\begin{center}
\AxiomC{$\{p\} E_i \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX_i \} \text{ for } i \in \mathbb{N}_n$}
\RightLabel{\scriptsize(INV)$\times n+1$}
\UnaryInfC{$\{p_i\} E_i \{p_{i+1}[l_i := \result] \} \text{ for } i \in \mathbb{N}_n$ \hspace{0.2cm} $(1)$}
\DisplayProof
\end{center}

Assuming that $\BaseTypeX_0 = \{C_1,...,C_k\}$, $(2)$ can be split using the DISJ rule and then derived from the
other $k$ premises of the $\restricted$-METH rule as follows

\begin{center}
\AxiomC{$\{p'''_j\} l_0.m(l_1,...,l_n) \{\TInv \wedge \llbracket \result \rrbracket \in \BaseTypeX'_j\} \text{ for } j \in \mathbb{N}^1_k$}
\RightLabel{\scriptsize(INV)$\times k$}
\UnaryInfC{$\{p''_j\} l_0.m(l_1,...,l_n) \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX'_j\} \text{ for } j \in \mathbb{N}^1_k$}
\RightLabel{\scriptsize(CONS)$\times k$}
\UnaryInfC{$\{p'_j\} l_0.m(l_1,...,l_n) \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\} \text{ for } j \in \mathbb{N}^1_k$}
\RightLabel{\scriptsize(DISJ)$\times k-1$}
\UnaryInfC{$\{p_{n+1}\} l_0.m(l_1,...,l_n) \{p \wedge \llbracket \result \rrbracket \in \BaseTypeX\}$ \hspace{0.2cm} $(2)$}
\DisplayProof
\end{center}

where $p'_j \equiv p \wedge \llbracket l_0 \rrbracket \in \{C_j\} \wedge \bigwedge\limits_{i=1}^n \llbracket l_i \rrbracket \in \BaseTypeX_i$,
$p''_j \equiv p \wedge \llbracket l_0 \rrbracket \in \{C_j\} \wedge \bigwedge\limits_{i=1}^n \llbracket l_i \rrbracket \in \BaseTypeX_{ij}$,
$p'''_j \equiv \TInv \wedge \llbracket l_0 \rrbracket \in \{C_j\} \wedge \bigwedge\limits_{i=1}^n \llbracket l_i \rrbracket \in \BaseTypeX_{ij}$ for $j \in \mathbb{N}^1_k$ and
for all $i \in \mathbb{N}_n, j \in \mathbb{N}^1_k: \BaseTypeX_i \subseteq \BaseTypeX_{ij}$ and $\BaseTypeX'_j \subseteq \BaseTypeX$.
The reason the INV rule can be applied like this is that $(\Var_L \setminus \{\result\}) \cap change(l_0.m(l_1,...,l_n)) = \emptyset$
and except for $\TInv$, the typing assertion $p$ can only contain references to local variables. \hfill $\Box$
\end{proof}

\todo{other rules}

% 
% \noindent RULE: $\restricted$-BLCK
% composed from BLCK, CONS, PASGN



==> sections/extensions.tex <==
\todo{POPL referee B: there is no motivation for why these extensions would
be valuable.  This section needs some kind of context to it.
}

%new
While the presented technique is complete relative to the Hoare logic and sufficient to conveniently verify many dynamically typed programs, the type safety verifier (see Section~\ref{sec:auto:type_safety_verifier}) used was intentionally simplistic to illustrate the minimum requirements for this role (see Section~\ref{sec:overview:semi-auto}). It can be expected that more powerful verifiers will increase the ratio of automation as well as allow more sophisticated typing annotations. Let us now discuss howto extend the technique to such verifiers.


\paragraph{Flow sensitivity}
Hoare Logic is flow sensitive. Flow-sensitive TI
transforms the program into single-assignment form, creating ``new'' variables after each assignment.
Mapping these ``virtual'' variables back to one in the translation is trivial.

\paragraph{Path sensitivity}
The conditional-example in Figure~\ref{fig:ex_cond} shows an example of how path-sensitivity can
be mapped into Hoare logic. When the TI types all paths separately, one
can also generate a separate proof attempt for each path, weaken their postconditions to a
disjunction of all cases and join the proof attempts together using the DISJ rule.

\paragraph{Context sensitivity}
In order to distinguish between different calls to a method, one can use the argument types
to distinguish contexts and construct method call assumptions of the form
%
\[\{c \wedge c_1 \vee ... \vee c_n\} l.m(v_1,...,v_k) \{ c_1 \rightarrow r_1 \wedge ... \wedge c_n \rightarrow r_n \}\]
%
where $c \equiv \llbracket l \rrbracket \in \{C\}, c_i \equiv \llbracket v_1 \rrbracket \in T_{1,i} \wedge ... \wedge \llbracket v_k \rrbracket \in T_{k,i}$,
and $r_i \equiv \llbracket \result \rrbracket \in T_i$ for $i \in \mathbb{N}^1_n$.
%
%%TODO{object sensitivity}



Context sensitivity

1. for a method call, derive
$\{\tau'_1 \vee ... \vee \tau'_k\} \PL{u}_0.\PL{m}(\PL{u}_1,...,\PL{u}_n) \{ \tau'_1 \wedge \llbracket \result \rrbracket \in T_1 \vee ... \vee \tau'_k \wedge \llbracket \result \rrbracket \in T_k \}$ where $\tau'_i$ are conjunctions of typing literals over the $\PL{u}_j$'s.

problem: the BLCK rule doe not allow mentioning local varibles except $\result$ in the postcondition. However, one can introduce logical variables $v_i$ such that $\PL{u}_i = v_i$ for all $i$ and express the property using the $v_i$. Using the INV rule this can be added to pre- and postcondition and an application of the CONS rule gives the desired result.

2. CONS rule allows to establish precondition $\tau'_i \rightarrow \tau'_1 \vee ... \vee \tau'_k$. INV rule and CONJ rule allow establishing $\{ \tau'_i \} \PL{u}_0.\PL{m}(\PL{u}_1,...,\PL{u}_n) \{ \tau'_i \wedge \llbracket \result \rrbracket \in T_i \}$ for all $i \in \mathbb{N}^1_k$.

$\Rightarrow$ while context sensitivity can be emulated using path sensitivity and the Hoare logic rules for method calls, it would be nice to add some support for this kind of reasoning (automatically adding the auxiliary variables, automatically applying the CONS and INV rules, etc.).

Object sensitivity

1. after their creation, establish a typing invariant for the desired objects of type $\{C\}$.

2. establich it as a global typing invariant

3. track the objects for which the invariant holds along all data-flows.

4. add another disjunct handling this case to method calls on object of type $\{C\}$. Handle it like context-sensitivity

$\Rightarrow$ while possible, this requires a lot of effort. Better: allow the type safety proof to introduce new subtypes $C' < C$. Then, the type inference algorithm can distinguish between $C$ and $C'$, takes care of the tracking along all dataflows, automatically discovers the types of $C'$'s instance variables and automatically establishes the global typing invariant. Also: 


==> sections/old.tex <==

\subsection{Outline}
The remainder of this paper is organized as follows:
the next Section~\ref{sec:motivation} will motivate the approach by illustrating it on several
small examples.

Then, the formal setting will be established by first introducing a dynamically typed model language
called \textbf{dyn} (Section~\ref{sec:language}) and giving a Hoare logic for it (Section~\ref{sec:HL}).

Afterwards, technical details will be given for each step of the procedure:
Section~\ref{sec:TI2HL} introduces the TI algorithm and a translation of its
results into Hoare logic proof attempts. The reason we call them proof attempts is that they may
not be valid proofs. This happens when the translation is used to translate inconsistent results.
Section~\ref{sec:HL2TI} introduces the idea of proof patches, small localized subproofs that can be
applied to such invalid proof attempts to repair them. Applying a patch usually yields more precise
type information that can in turn be used by the TI to compute a more precise typing
for the remaining program. This yields the previously mentioned iterative back-and-forth procedure between
automatic TI and manual construction of proof patches.
Section~\ref{sec:layer} then gives the details on how to use the obtained type information to establish
a layer of abstraction, separating typing problems from other correctness issues and allowing
the direct use of a statically typed assertion language to reason about states of
dynamically typed programs.

In the end,
Section~\ref{sec:Extensions} discusses a number of extensions for applying this methodology
to more sophisticated TI algorithms,
Section~\ref{sec:related_work} summarizes related work and Section~\ref{sec:conclusion} concludes
and discusses future work.

\section{Motivation}
\label{sec:motivation}














\ifx \version\extended
\subsection{Correctness}
\label{sec:HL-soundness}

The following section will introduce an object-oriented programming language along with
a sound and complete Hoare logic. Both are fairly standard. A version without object creation
and using an assertion language without quantification over objects is proven sound and complete
in \cite{AptDeBoerOlderog2012}.
How to extend the logic to allow both
object creation and
quantification over objects while retaining soundness and completeness
is discussed in \cite{DeBoerPierik2003}.

\subsection{Target Language: Object-Oriented Programs}

\begin{figure}
$\pi \in \mathit{Prog}^{oo} ::= \Vector{\mathit{meth}} \text{ } S$

$\mathit{meth} \in \mathit{Meth}^{oo} ::= \PL{m}(\Vector{u}) \{ S \}$

$S \in \mathit{Stmt}^{oo} ::= \PL{skip} \mid \PL{u} := e \mid \PL{x} := e \mid e.\PL{m}(\Vector{e}) \mid \PL{u} := \PL{new}$

\hspace{1.3cm}$\mid \PL{if } e \PL{ then } S \PL{ else } S \PL{ fi} \mid \PL{if } e \rightarrow S \PL{ fi} \mid S; S$

\hspace{1.3cm}$\mid \PL{while } e \PL{ do } S \PL{ done} \mid \PL{begin local } \Vector{\PL{u}} := \Vector{e}; S \PL{ end}$

$e \in \mathit{Expr}^{oo} ::= \PL{null} \mid \PL{this} \mid \PL{u} \mid \PL{x} \mid e = e \mid op(\Vector{e})$

$\PL{m} \in \Method^{oo}, \PL{u} \in \Var^{oo}_L, \PL{x} \in \Var^{oo}_I$

\caption{\label{fig:oo_syntax}Syntax of object-oriented programs}
\end{figure}

The syntax of object-oriented programs is given in Figure~\ref{fig:oo_syntax}. As there are
no classes, a program consists of a set of methods $\Method^{oo}$ and a main statement $S$.
The set of variables $\Var^{oo} = \Var^{oo}_L \uplus \Var^{oo}_I$ contains both local and
instance variables.

$op(\Vector{e})$ represents a number of predefined side-effect-free $n$-ary operations. These can be
defined arbitrarily. However, for the expressions of the programming language to be a subset of the
logical expressions used in the assertion language, the same operations must be used. In particular,
equality is non-strict with respect to $\Vnull$ values.

\subsection{Semantics}

The semantics of object-oriented programs is given in Figure~\ref{fig:semantics_OO}.
$E$ denotes the empty program and $E;S \equiv S$ for all statements $S$.

The value domain $\mathcal{D}^{oo} = \bigcup_{t \in \mathcal{T}} \mathcal{D}_{t}$ with
$\mathbf{object} \in \mathcal{T}$ is used to account for different value types:
program variables are
typed and may be of any basic type $t \in \mathcal{T}$. Logical variables (used in the assertion
language) can also be of a sequence type $t^*$ for $t \in \mathcal{T}$ which means they represent
a finite sequence of elements of type $t$.
For this paper we use $\mathcal{T} = \{ \mathbf{object}, \mathbb{N}, \mathbb{B} \}$.
The programming language is statically typed. It is thus f.i. statically ensured
that in assignments $\PL{u} := e$ the type of the local variable $\PL{u}$
coincides with the type of the expression
$e$ and that the conditions of conditionals, loops and failure statements are boolean.

However, note that object-oriented programs do
not support classes. All methods in $\Method^{oo}$ can be called on any object and all instance
variables in $\Var^{oo}_I$ exist for any object. While failure at runtime is possible
(calling a method on $\Vnull$), type errors are not.
 
We omit the definitions for states, state update and expression evaluation ($\sigma(e)$)
as they are standard.

Furthermore, we model object creation as object activation and introduce
a special instance variable $\mathit{active}$ of type $\mathbb{B}$,
an infinite sequence of distinct objects $o_1,o_2,...$ that are initially inactive
($o_i.\mathit{active} = \mathit{false}$ for all $i \in \mathbb{N}$) as well as 
a function $\creation: \Sigma \mapsto \mathcal{D}_{\mathbf{object}}$ mapping
a proper state $\sigma$ to the object $o_i$
with the least index $i$ that is inactive in $\sigma$.

% two special variables $\store$ and $\Vcount$.
% Both are allowed to appear in neither program statements nor assertions. $\store$ is an array variable of type
% $\mathbb{N} \rightarrow \mathbf{object}$ and $\Vcount$ is a variable of type $\mathbb{N}$. $\store$ is assumed
% to be injective:
% %
% \[ \forall i,j \bullet i \not= j \rightarrow \store[i] \not= \store[j] \]
% %
% which is possible as $\mathcal{D}_{\mathbf{object}}$ is unbounded. We call all objects $o$ with
% $\exists i \leq \Vcount \bullet o = \store[i]$ active and all others inactive.
A proper state $\sigma$ is
called consistent when the objects $\PL{this}$ and $\Vnull$ are active and all
local object variables as well as all instance object variables
of active objects also refer to active objects.

The notions of correctness underlying the Hoare logic introduced in the next section only consider
consistent states.

\begin{figure}
 \begin{enumerate}
 \item $ \langle \PL{skip}, \sigma \rangle  \step  \langle E,\sigma \rangle $
 
 \item $ \langle \PL{v} := e, \sigma \rangle  \step  \langle E, \sigma[\PL{v} := \sigma(e)] \rangle$ where $\text{v} \in \Var^{oo}$
 
% \item $ \langle \PL{x} := e, \sigma \rangle  \step  \langle E, \sigma[\PL{x} := \sigma(e)] \rangle$

 \item $ \langle \Vector{u} := \Vector{e}, \sigma \rangle  \step  \langle E, \sigma[\Vector{u} := \sigma(\Vector{e})] \rangle $
       where $\Vector{u} \in {{\Var}^{oo}_L}^+$
       
 \item \AxiomC{$ \langle S_1, \sigma \rangle  \step  \langle S_2, \tau \rangle $}
       \UnaryInfC{$ \langle S_1; S, \sigma \rangle  \step  \langle S_2; S, \tau \rangle $}
       \DisplayProof
 \item $ \langle \PL{if } e \PL{ then } S_1 \PL{ else } S_2 \PL{ fi}, \sigma \rangle  \step  \langle S_1, \sigma \rangle $ where $\sigma \models e$
 \item $ \langle \PL{if } e \PL{ then } S_1 \PL{ else } S_2 \PL{ fi}, \sigma \rangle  \step  \langle S_2, \sigma \rangle $ where $\sigma \models \neg e$
 \item $ \langle \PL{while } e \PL{ do } S \PL{ od}, \sigma \rangle  \step  \langle S; \PL{while } e \PL{ do } S \PL{ od}, \sigma \rangle $ where $\sigma \models e$
 \item $ \langle \PL{while } e \PL{ do } S \PL{ od}, \sigma \rangle  \step  \langle E, \sigma \rangle $ where $\sigma \models \neg e$
 \item $ \langle \PL{begin local } \Vector{\PL{u}} := \Vector{e}; S \PL{ end}, \sigma \rangle  \step  \langle \Vector{\PL{u}} := \Vector{e}; S; \Vector{\PL{u}} := \sigma(\Vector{\PL{u}}), \sigma \rangle $
 \item $ \langle e_0.\PL{m}(\Vector{e}), \sigma \rangle  \step$\newline
       $ \langle $if $e_0 \not= \Vnull \rightarrow$ begin local $ \PL{this}, \Vector{\PL{u}} := e_0, \Vector{e}; S $ end fi$, \sigma \rangle $

       where $\PL{m}(\Vector{\PL{u}}) \{ S \} \in \Method^{oo}$
%  \item $ \langle s.m(\Vector{t}), \sigma \rangle  \step  \langle \emptyP, \mathbf{fail} \rangle $
% 
%        where $\sigma \models s = \Vnull$
% does not exist in oo-programs
%  \item $ \langle s.m(\Vector{t}), \sigma \rangle  \step  \langle \emptyP, \mathbf{typeerror} \rangle $
% 
%        where $\sigma \models s \not= \Vnull$ and $m(\Vector{u}) :: S \not\in D$

 \item $ \langle $if $e \rightarrow S$ fi$, \sigma \rangle  \step  \langle S, \sigma \rangle $, where $\sigma \models e$,
 \item $ \langle $if $e \rightarrow S$ fi$, \sigma \rangle  \step  \langle E, \mathbf{fail} \rangle $, where $\sigma \models \neg e$,

% \item $ \langle $if$_\tau$ $e \rightarrow S$ fi$, \sigma \rangle  \step  \langle S, \sigma \rangle $, where $\sigma \models e$,
% \item $ \langle $if$_\tau$ $e \rightarrow S$ fi$, \sigma \rangle  \step  \langle E, \mathbf{typeerror} \rangle $, where $\sigma \models \neg e$,
 
 \item $ \langle \PL{u} := \PL{new}, \sigma \rangle  \step$\newline
       $\langle E, \sigma[o.\mathit{active} := \mathit{true}][\PL{u} := o] \rangle$ where $o = \creation(\sigma)$
\end{enumerate}
\caption{\label{fig:semantics_OO} Structural operational semantics of OO-programs}
\end{figure}

\subsection{Hoare Logic}

The assertion language is the same as for dyn.
\todo{arrays -> aliasing}
\todo{classes -> object creation}

The Hoare Logic for object-oriented programs is as follows.
The rules SEQ, CONS as well as the auxiliary rules DISJ, CONJ, $\exists$-INT and SUBST
are the same as the ones given in Section~\ref{sec:HL}.

\noindent AXIOM: SKIP

\begin{center}
$\{p\} \PL{skip} \{p\}$
\end{center}

\noindent RULE: ASGN (both normal and instance variables)
%
\begin{center}
\AxiomC{$\{p[\PL{v} := e]\} \PL{v} := e \{p\}$ \hspace{1cm} where $\PL{v} \in \Var^{oo}$}
\DisplayProof
\end{center}
%

\noindent RULE: COND
%
\begin{center}
\AxiomC{$\{p \wedge e\} S_1 \{q\}$}
\AxiomC{$\{p \wedge \neg e\} S_2 \{q\}$}
\BinaryInfC{$\{p\}$ if $e$ then $S_1$ else $S_2$ fi $\{q\}$}
\DisplayProof
\end{center}

\noindent RULE: LOOP
%
\begin{center}
\AxiomC{$\{p \wedge e \} S \{p\}$}
\UnaryInfC{$\{p\}$ while $e$ do $S$ done $\{p \wedge \neg e\}$}
\DisplayProof
\end{center}

\noindent RULE: FAIL
%
(partial correctness \StrongPC{+strong} )
%
\begin{center}
\AxiomC{$\mStrongPC{p \rightarrow e}$}
\AxiomC{$\{p \wedge e\} S \{q\}$}
\BinaryInfC{$\{p\}$ if $e \rightarrow S$ fi $\{q\}$}
\DisplayProof
\end{center}

\noindent RULE: PASGN
%
\begin{center}
$\{p[\Vector{\PL{u}} := \Vector{e}]\} \Vector{\PL{u}} := \Vector{e} \{p\}$ \hspace{1cm} where $\Vector{\PL{u}} \in {\Var^{oo}_L}^+$
\end{center}

\noindent RULE: BLCK
%
\begin{center}
\AxiomC{$\{p\} \Vector{\PL{u}} := \Vector{e}; S \{q\}$}
\RightLabel{ where $\{\Vector{\PL{u}}\} \cap \free(q) = \emptyset$}
\UnaryInfC{$\{p\}$ begin local $\Vector{\PL{u}} := \Vector{e}; S \text{ end} \{q\}$}
\DisplayProof
\end{center}

\noindent RULE: REC
%
(partial correctness \StrongPC{+strong} )
%
\begin{center}
\AxiomC{$\begin{matrix}
          A \vdash \{p\} S \{q\}, \\
          A \vdash \{p_i\} \PL{begin local this}, \Vector{\PL{u}_i} := \PL{l}_i,\Vector{e_i}; S_i \PL{ end} \{q_i\}, i \in \mathbb{N}^1_n \\
          \mStrongPC{p_i \rightarrow \PL{l}_i \not= \PL{null}, i \in \mathbb{N}^1_n}
         \end{matrix}$}
       
\UnaryInfC{$\{p\} S \{q\}$}
\DisplayProof
\end{center}
%
where $\PL{m}_i(\Vector{\PL{u}_i}) \{ S_i \} \in \Method^{oo}$ for $i \in \mathbb{N}^1_n$ and \newline
$A = \{ \{\PL{p}_1\} \PL{l}_1.\PL{m}_1(\Vector{e_1}) \{q_1\}, ..., \{p_n\} \PL{l}_n.\PL{m}_n(\Vector{e_n}) \{q_n\} \}$.

\vspace{0.2cm}
\noindent AXIOM: NEW
%
\begin{center}
$\{p[\PL{u} := \PL{new}]\} \PL{u} := \PL{new} \{p\}$
\end{center}

\subsection{Auxiliary Rules}
\label{sec:aux_rules}

\noindent Auxiliary RULE: INV

\begin{center}
\AxiomC{$\{r\} S \{q\}$}
\UnaryInfC{$\{p \wedge r\} S \{p \wedge q\}$}
\DisplayProof
\end{center}
where $\free(p) \cap (change(\Method^{oo}) \cup change(S)) = \emptyset$ and
$p$ does not contain quantification over objects.

\subsection{Dyn as an Extension of OO-Programs}

We now 
%start from the object-oriented programs described in \cite{AptDeBoerOlderog2012} and
describe a transformation from \textbf{dyn} programs to object-oriented programs which is then
used to establish soundness and completeness of the Hoare logic given for dyn.

\subsubsection{Transformation}

For our transformation, direct access to return values will be necessary. We therefore introduce
a special local variable $\PL{r} \in \Var^{oo}_S$ that is not used in the \textbf{dyn} program to be
transformed but may be
accessed like any other variable in the resulting simple OO-program.
The transformation will ensure that after executing a resulting OO-statement, $\PL{r} = \result$ holds.

% dyn
% - hierarchy of classes, each with a set of methods
% - instance variables of a class are those assigned in its constructor, init
% - disjoint domains D_C for every class C
% - null is only element \in D_{NullClass}
% oo
% - no classes
% - set of methods (can be called on every object)
% - set of instance variables (for all objects)

In dyn-programs, there is a hierarchy of classes each with its set of methods.
%The classes have disjoint domains ($\mathcal{D}_C = \{ o \in \mathcal{D} | o.@\mathbf{c} = o_C \}$ for each class $C$) populated by their respective instances.
%The $\Vnull$ value is the only instance of class $\mathbf{Nullclass}$.
A classes instance variables are those used in its methods.

Object-oriented programs on the contrary do neither
support any classes nor distinguish any values of type object. There is only a global set of methods $\Method^{oo}$
which can be called on any object. Also, the full set $\IVarOO$ of instance variables can be accessed on
any object.

To model the behavior of \textbf{dyn} programs with respect to classes, we reuse the \textbf{dyn} mechanism
by setting the instance variable $o.@\mathbf{c}$ to $\oC_C$ whenever $o$ is an instance of $C$.

We start by defining a function $\Theta: \Var \mapsto \Var^{oo}$ mapping \textbf{dyn} variables to OO-variables.
%
\begin{align*}
\Theta(\result) & = \PL{r}, \Theta(\PL{v}) = \PL{v} \text{ for } \PL{v} \in \Var \setminus \{\result\}, \\
\VarOO & = \Theta(\Var_L) \cup \{\Vcount, \store, l_1,l_2,...\}, \IVarOO = \Theta(\Var_I)
\end{align*}
%
The handling of the special variables will be explained below.

We now overload $\Theta: \Sigma_{dyn} \mapsto \Sigma_{oo}$ to also map dyn-states $\sigma$ into
states of simple object-oriented programs $\Theta(\sigma)$.
%
% mapping states:
% - making the partial functions total
% - mapping the objects from $\mathcal{D}$ to $\mathcal{D}_{oo}$
%
\begin{itemize}
 \item $\Theta(\mathbf{fail}) = \mathbf{fail}$
 \item $\Theta(\mathbf{typeerror}) = \mathbf{typeerror}$
 \item $\Theta(\sigma) = \sigma'$
 
 where $\sigma' = (\sigma'_E, \sigma'_H) \in \Sigma_{oo}$ can be derived from the proper state $\sigma = (\sigma_E, \sigma_H) \in \Sigma_{dyn}$ as follows
% 
\begin{itemize}
  \item mapping all dyn-objects $o \in \mathcal{D}$ to OO-objects
        $\Theta(o) \in \mathcal{D}_{\mathbf{object}}$.
        
  \item deriving a total environment $\sigma'_E$ from the partial $\sigma_E$ by assigning $\Vnull$ to
        all variables $v \in \VarOO \setminus dom(\sigma_E)$.
        
  \item making all local states $\sigma_H(o)$ total by assigning $\Vnull$ to each instance variable
        $@v \in \IVarOO \setminus dom(\sigma_H(o))$ for all objects $o$.
        In particular, instance variables of inactive objects are all set to $\Vnull$.

% not neccessary
%   \item substituting the instance variable $@\mathbf{c}$ with
%         $\sigma(o)(@\mathbf{c}) = \oC_C$ by
%         an instance variable $\mathbf{c}$ of type num such that $\sigma'(\Theta(o))(\mathbf{c}) = N_C$
%         for all active objects $o$.
\todo{replace $N_C$ by $\oC_C$ and $o.\mathbf{c}$ by $o.@\mathbf{c}$ everywhere}

  \item Add the special global variables $\Vcount$ of type $\mathbb{N}$ and $\store$
        of type $\mathbb{N} \rightarrow \mathbf{object}$. $\store$ should reference all objects,
        active or inactive, in the same order as the sequence $o_1,o_2,...$ defined in
        Section~\ref{sec:dyn_semantics}, that is $\store[i] = \Theta(o_i)$ for all $i \in \mathbb{N}$.
        When $\creation(\sigma) = o_k$, then $\Vcount = k-1$. Without loss of generality, we
        assume that there are no
        variables named $\Vcount$ or $\store$ in the \textbf{dyn} program to be translated.
        
  \item instead of $\result$, add a special local variable $\PL{r}$ of type $\mathbf{object}$ such that
        $\sigma'(\PL{r}) = \Theta(o)$ iff $\sigma(\result) = o$
         and a sequence of simple variables
        $l_1,l_2,...$ of type $\mathbf{object}$ that can be used by the transformation as fresh
        variables. Map these variables to $\Vnull$. We consider proper states of object-oriented programs
        equivalent when they are equivalent on all variables except $\{l_1, l_2,...\}$.
 \end{itemize}
\end{itemize}
%
Next, we extend the mapping $\Theta$ to map statements of dyn-programs to statements of simple OO-programs.
%
\begin{itemize}
 \item $\Theta(S_1; S_2) \equiv \Theta(S_1); \Theta(S_2)$
 \item $\Theta(\PL{null}) \equiv \PL{r} := \PL{null}$
 \item $\Theta(\PL{u}) \equiv \PL{r} := \PL{u}$
 \item $\Theta(\PL{@x}) \equiv \PL{r} := \PL{@x}$
 \item $\Theta(\PL{this}) \equiv \PL{r} := \PL{this}$
 \item $\Theta(\PL{v} := E) \equiv \Theta(E); \PL{v} := \PL{r}$
 \item $\Theta(\PL{@v} := E) \equiv \Theta(E); \PL{@v} := \PL{r}$

 \item $\Theta(E_0.\PL{m}(E_1,...,E_n)) \equiv$\newline
 \hspace*{0.5cm}$\Theta(E_0); l_0 := \PL{r}; ...; \Theta(E_n); l_n := \PL{r}; \Theta(l_0.\PL{m}(l_1,...,l_n))$\newline
 where $l_i$ are fresh for all $i \in \mathbb{N}_n$.

 \item $\Theta(l_0.m(l_1,...,l_n)) \equiv$ if $l_0 \not= \Vnull \rightarrow S_k$ fi\newline
 where $S_k$ is defined inductively as follows
 \begin{itemize}
  \item $S_0 =$ if$_\tau$ $\mathit{false} \rightarrow \PL{skip}$ fi
  \item $S_i =$ if $l_0.\PL{@}\mathbf{c} = \oC_{C_i}$ then $l_0.\PL{m@C}_i(l_1,...,l_n, \Vector{\PL{null}})$ else $S_{i-1}$ fi
 \end{itemize}
 where $\{C_1,...,C_k\}$ is the set of classes supporting a method $\PL{m}$ of arity $n$ and
 $\Vector{\PL{null}}$ is a
 sequence of $|\Theta(\Var_L \setminus \Var_S)|-n$ $\Vnull$-constants.

 \item $\Theta($new $C(E_1,...,E_n)) \equiv \Theta(\mathbf{new}_C.\mathit{init}(E_1,...,E_n))$

 \item $\Theta(\mathbf{new}_C) \equiv \PL{r} := \PL{new}; \PL{r}.\PL{@}\mathbf{c} := \oC_C$
 
 \item $\Theta($if $E$ then $S_1$ else $S_2$ end$) \equiv$\newline
 \hspace*{0.5cm}$\Theta(E);$ if $\PL{r} \not= \PL{null} \rightarrow$ if$_\tau$ $\PL{r}.\PL{@}\mathbf{c} = \oC_{\mathit{bool}} \rightarrow r.to\_ref()$ fi fi$;$ if $\PL{r} \not= \PL{null}$ then $\Theta(S_1)$ else $\Theta(S_2)$ fi
 
 \item $\Theta($while $E$ do $S$ done$) \equiv$\newline
 \hspace*{0.5cm}$\Theta(E); $ if $\PL{r} \not= \PL{null} \rightarrow$ if$_\tau$ $\PL{r}.\PL{@}\mathbf{c} = \oC_{\mathit{bool}} \rightarrow r.to\_ref()$ fi fi$;$ while $\PL{r} \not= \PL{null}$ do $\Theta(S); \Theta(E);$ if $\PL{r} \not= \PL{null} \rightarrow $ if$_\tau$ $\PL{r}.\PL{@}\mathbf{c} = \oC_{\mathit{bool}} \rightarrow \PL{r.to\_ref}()$ fi fi od; $\PL{r} := \PL{null}$

 \item $\Theta(\Vector{\PL{u}} := \Vector{\PL{l}}) \equiv \Theta(\Vector{\PL{u}}) := \Theta(\Vector{\PL{l}})$

 \item $\Theta($begin local $\Vector{\PL{u}} := \Vector{\PL{l}}; S$ end$) \equiv$\newline
   \hspace*{0.5cm}begin local $\Theta(\Vector{\PL{u}} := \Vector{\PL{l}}); \Theta(S)$ end
\end{itemize}
%
%
% $\Theta(\Vnull) \equiv \Vnull$
% 
% $\Theta(x) \equiv x$ for every local variable $x$.
% 
% $\Theta(@x) \equiv @x$, $@x$ on the left-hand-side denoting an OO-instance variable and on the right-hand-
% side a dyn-instance variable.
% 
% $\Theta(\this) = \this$
% 
% This mapping satisfies the following properties
% 
% \begin{lemma}
% For all proper states $\sigma$ the following hold.
% \begin{itemize}
%  \item For all expressions $s$, \[\sigma(s) = \Theta(\sigma)(\Theta(s)).\]
%  \item For all instance variables @u and objects d
%  \[\Theta(\sigma[@u := d]) = \Theta(\sigma)[\Theta(@u) := d].\]
% \end{itemize} 
% \end{lemma}
%
%
%
% Now, we can extend the mapping to restricted dyn-statements:
% 
% \begin{definition} \textbf{(Translation)} $\Theta: S_{rdyn} \mapsto S_{oo}$ is defined inductively over the structure of
% restricted \textbf{dyn} statements.
% 
% \begin{itemize}
%  \item $\Theta(S_1;S_2) \equiv \Theta(S_1); \Theta(S_2)$
%  \item $\Theta(r := E) \equiv r := \Theta(E)$
%  \item $\Theta(l := r) \equiv l := r$
%  \item $\Theta(@v := r) \equiv @v := r$
% % \item $\Theta(r := l_0.m(l_1,...,l_n)) \equiv l_0.m(l_1,...,l_n)$ %TODO{old}
%  \item $\Theta(r := l_0.m(l_1,...,l_n)) \equiv$ if $l_0 \not= \Vnull$ then $S_n$ else $\mathbf{fail}$ end
% 
%  where $S_n$ is defined inductively as follows
%  \begin{itemize}
%   \item $S_0 = \textbf{typeerror}$
%   \item $S_i =$ if $l_0.\mathbf{c} = N_{C_i}$ then $l_0.m@C_i(l_1,...,l_n)$ else $S_{i-1}$ fi
%  \end{itemize}
%  where $\{C_1,...,C_n\}$ is the set of classes supporting a method $m$ of arity $n$.
%  
%  \item $\Theta(r := $ new $C(l_1,...,l_n)) \equiv r := \mathbf{new}; r.@\mathbf{c} := \oC_C; r.init(l_1,...,l_n)$
%  \item $\Theta(r := $ if $l$ then $S_1$ else $S_2$ end$) \equiv$\newline
%  \hspace*{1cm} $l.to\_ref();$ if $r \not= \Vnull$ then $\Theta(S_1)$ else $\Theta(S_2)$ fi
%  \item $\Theta(r :=$ while $l$ do $S$ done$) \equiv$\newline
%  \hspace*{1cm} $l.to\_ref();$ while $r \not= \Vnull$ do $\Theta(S); l.to\_ref()$ od$; r := \Vnull$
%  \item $\Theta(\Vector{l} := \Vector{l'}) \equiv \Vector{l} := \Vector{l'}$
%  \item $\Theta($begin local $\Vector{u} := \Vector{l}; S$ end$) \equiv $begin local $\Vector{u} := \Vector{l}; \Theta(S)$ end
% \end{itemize}
% \end{definition}
%
Finally, we transform every method declaration in the restricted dyn-program
%
\[ \PL{method m}(\PL{u}_1,...,\PL{u}_n) \{ S \} \in \Method_C \]
%
into a method declaration in the OO-proram
%
\[ \PL{m@C}(\PL{u}_1,...,\PL{u}_n, \Vector{\PL{l}}) \{ \Theta(S) \} \]
%
where $\{\Vector{\PL{l}}\} = \Theta(\Var_L \setminus \Var_S) \setminus \{\PL{u}_1,...,\PL{u}_n\}$.

Note that any such method will automatically store its return value in $\PL{r}$ since its body is a converted
\textbf{dyn} statement. Since $\PL{r}$ is a special variable, it is not overwritten by the block statement
resulting from a method invocation. Hence after returning from a method call, the result will still be
stored in $\PL{r}$.
A similar argument holds for the branches of an if-statement. Thus neither method calls nor conditionals
must explicitly store their result in $\PL{r}$.

\subsubsection{Correctness of the transformation}
%
\begin{lemma} \label{transformation_lemma_for_Theta} \textbf{(Transformation)} For all
dyn-programs $S$, all sets of classes $\Class$ with method declarations $\Method_C$, all proper states
$\sigma$, and all proper or $\mathbf{fail}$ or $\mathbf{typeerror}$ states $\tau$,
%
\[ \langle S,\sigma \rangle \mstep  \langle \emptyP,\tau \rangle \text{ iff } \langle \Theta(S),\Theta(\sigma) \rangle \mstep \langle E,\Theta(\tau) \rangle \]
\end{lemma}
%
\begin{proof}
 By comparing the outcome $\tau$ of $S$ for a proper state $\sigma$ with the outcome $\tau'$ of $\Theta(S)$
 for $\Theta(\sigma)$ and checking that $\tau' = \Theta(\tau)$ for all cases. $\Box$
 \todo{give the cases for method call and object creation}
\end{proof}
%
%re-proof done%
%2do:
% 
% ok:
% S ::= S;S, null, v, @v, this, v := E, @v := E, s.m(E), begin, pasgn, while, new C(E)
%
Finally, the following theorem establishes correctness of $\Theta$ as a homomorphism. For this theorem
we extend $\Theta$ to sets of states in the obvious way.
%
\begin{theorem}
\label{correctness_of_Theta}
 \textbf{(Correctness of $\Theta$)} For all dyn-programs $S$, all sets of classes $\Class$ with
 method declarations $\Method_C$, and all proper states $\sigma$ the following holds:

\begin{itemize}
 \item $ \Theta(\mathcal{M}\llbracket S \rrbracket(\sigma)) = \mathcal{M}\llbracket \Theta(S) \rrbracket(\Theta(\sigma))$
\end{itemize}
%
where $S$ is considered in the context of the set $\Class$ of \textbf{dyn} class declarations (each with its
corresponding method declarations $\Method_C$) and the corresponding object-oriented program $\Theta(S)$ in
the context of the set of method declarations $\Theta(\bigcup_{C \in \Class}\Method_C)$.
\end{theorem}
%
\textbf{Proof.} Theorem~\ref{correctness_of_Theta} is a direct consequence of Lemma~\ref{transformation_lemma_for_Theta}.


% \subsection{correctness of restriction}
% %TODO{merge with previous section}
% % $\Gamma(\sigma) = \sigma[r := \result]$  (should never overwrite anything as $r$ is not used in the
% % program to be transformed)
% 
% Let $l_1,l_2,...$ be a sequence of variables that are not used anywhere in the program to be restricted and
% used by the $\Gamma$-translation whenever a fresh variable is needed.
% 
% We use $\check{\sigma}$ to denote the proper state $\sigma$ with all mappings to $r, l_1, l_2,...$ removed.
% 
% \begin{lemma}
% \label{transformation_lemma_for_Gamma}
% $\forall S,\sigma,\tau$
% 
% $\bullet  \langle S, \check{\sigma} \rangle  \mstep  \langle \emptyP,\check{\tau} \rangle $ iff $ \langle \Gamma(S), \sigma \rangle  \mstep  \langle \emptyP,\tau \rangle $
% \end{lemma}
% 
% \textbf{Proof.} By induction over the structure of \textbf{dyn} statements.
% %ok: null,v,@v,this, s;s, v := E, @v := E, e.m(e1,...,en),new C(e1,...,en), if, while
% 
% The only interesting case being Sequential Composition: $\Gamma(S_2)$ is executed in some state $\Gamma(\tau)$ instead of $\tau$, which
% is identical top $tau$ except for the added variable $r$. Therefore, if the first statement of $\Gamma(S_2)$
% would be of the form $l := r$, its behaviour could differ from when it is executed in state $\tau$. However,
% $\Gamma(S_2)$ is a translated \textbf{dyn} program and the $\Gamma$-translation will never yield a program beginning
% with $l := r$.
% 
% 
% \begin{theorem}
% $\forall S,\sigma$
% 
% $\bullet \Gamma(\mathcal{M}\llbracket S \rrbracket(\sigma)) = \mathcal{M}\llbracket \Gamma(S) \rrbracket(\Gamma(\sigma))$
% \end{theorem}
% 
% \textbf{Proof.} direct consequence of Lemma~\ref{transformation_lemma_for_Gamma}


\subsection{Translating Proofs}

We extend $\Theta$ to assertions. Without loss of generality, we assume that there are no
variables named $\Vcount$ or $\store$ or $\PL{r}$ in the assertions to be translated.
%
\[ \Theta(p) \equiv \Theta'(p[\result := \PL{r}]) \]
%
Where $\Theta'$ structuarally traverses the parse tree of a given assertion $A$, replacing
object equivalences as follows:
\begin{itemize}
% \item $\Theta'(\forall v \bullet A) \equiv \forall v \bullet \Theta'(A)$
% \item $\Theta'(\exists v \bullet A) \equiv \exists v \bullet \Theta'(A)$
 \item $\Theta'(L_1 = L_2) \equiv \Theta'(L_1) = \Theta'(L_2) \wedge \Theta''(L_1) \wedge \Theta''(L_2)$\newline
       where $L_1,L_2$ are of type $\mathbf{object}$.
\end{itemize}
%
All other cases are straightforward. $\Theta''$ structurally traverses the parse tree of a given
logical expression of type $\mathbf{object}$, returning $\mathit{true}$ on the leaves. The only interesting
cases are the following
%      
\begin{itemize}
 \item $\Theta''(L.\PL{@v}) \equiv \Theta''(L) \wedge L \not= \PL{null} \wedge$\newline
       \hspace*{2cm}$L.\PL{@}\mathbf{c} = \oC_{C_1} \vee ... \vee L.\PL{@}\mathbf{c} = \oC_{C_n}$\newline
       where $\{C_1,...,C_n\} = \{ C \mid \PL{@v} \in \Var_C \}$.
 \item $\Theta''($if $B$ then $L_1$ else $L_2$ fi$) \equiv$\newline
       \hspace*{1cm}$\Theta'(B) \wedge \Theta''(L_1) \vee \neg \Theta'(B) \wedge \Theta''(L_2)$\newline
       where $L_1,L_2$ are of type $\mathbf{object}$.
\end{itemize}
%
The object equivalence $\PL{x.@a} = \PL{null}$ is thus replaced by
$\PL{x} \not= \PL{null} \wedge \PL{x.@}\mathbf{c} = \oC_A \wedge \PL{x.@a} = \PL{null}$
assuming that the class $\PL{A}$ is the only one having an instance variable $\PL{@a}$. This is
neccessary to handle cases where $\sigma \not\models \PL{o.@v} = \PL{null}$ because
$\PL{@v} \not\in dom(\sigma(\PL{o}))$, but $\Theta(\sigma) \models \PL{o.@v} = \PL{null}$ as the translation
$\Theta$ initializes $\PL{@v}$ to $\Vnull$.
%
%
\begin{lemma} \textbf{(Assertion)}
\label{assertion_lemma}
 For all assertions $p$ and all proper states $\sigma$
 \[ \sigma \models p \text{ iff } \Theta(\sigma) \models \Theta(p). \]
\end{lemma}
%
\textbf{Proof.} By induction over the structure of $p$.
%
\begin{lemma} \textbf{Distributivity with Variable Substitution}\newline\todo{is ``Distributivity'' the right term here?}
 \label{lem:dist_subst_theta}
 For all assertions $p$ and variables $\PL{v},\PL{u} \in \Var$
 \[ \Theta(p[\PL{v} := \PL{u}]) \equiv \Theta(p)[\Theta(\PL{v}) := \Theta(\PL{u})] \]
\end{lemma}
%
\textbf{Proof.} By induction over the structure of $p$.
%
\begin{lemma} \textbf{Distributivity with Object Creation}\newline
 \label{lem:dist_new_theta}
 For all pure assertions $p$ and variables $\PL{v} \in \Var_L$
 \[ \Theta(p[\PL{v} := \mathbf{new}_C]) \equiv \Theta(p)[\PL{v.@}\mathbf{c} := \oC_C][\PL{v} := \mathbf{new}] \]
\end{lemma}

%
\begin{corollary} \textbf{(Translation I)}
 For all correctness formulas $\{p\} S \{q\}$ where S is a dyn-program,
 \[ \models \{p\} S \{q\} \text{ iff } \models \{\Theta(p)\} \Theta(S) \{\Theta(q)\} \]
and
 \[ \models_{sp} \{p\} S \{q\} \text{ iff } \models_{sp} \{\Theta(p)\} \Theta(S) \{\Theta(q)\} \]
\end{corollary}
%
\textbf{Proof.} Follows directly from the Assertion Lemma~\ref{assertion_lemma} and the correctness of
$\Theta$ (Theorem~\ref{correctness_of_Theta}).

%TODO{translate proofs of dyn-programs to assertions of oo-programs (later, when completeness is needed)}

As a preparation for the translation of proofs, we first distinguish the proof rules of the proof system for object-oriented programs into
adaption rules, which are
the consequence rule and the auxiliary rules
(which are similar to the ones given in Section~\ref{sec:aux_rules}) and structural rules
(all other rules). The reason for this distinction is that applications of structural rules are
always associated with a specific syntactic element and thus have a ``fixed place'' within
proofs containing this element while the position of adaption rule applications can be changed
as shown by the following theorem

\todo{give proof system for OO-programs}
\todo{change this from SPO+ to the given proof system for OO-programs}
\begin{theorem} \textbf{Reordering of Proof Rules}
\label{thm:reordering}

 For every proof in the proof system $\mathrm{SPO}^+$ for strong partial correctness of object-oriented
 programs, there exists an equivalent proof not containing any applications of adaption rules within
 continuous proof-subtrees otherwise only containing applications of the rules for sequential composition,
 conditional and failure (both kinds).
\end{theorem}

A proof of Theorem~\ref{thm:reordering} can be found in the appendix.\todo{add proof}

\begin{theorem} \textbf{Elimination of Proof Rules}
 \label{thm:elimination}
 For every proof in the proof system $\mathrm{SPO}^+$ for strong partial correctness, consisting of
 applications of only a single (structural) axiom (ASGN, PASGN, CONST, VAR or IVAR) and any number of
 adaption rule applications,
 there exists an equivalent proof consisting of only one application of the respective axiom, and
 an application of the CONS rule.
 \todo{check if this also holds for NEW}
\end{theorem}
\todo{provide a table mapping rule names to rule numbers is the original paper}

A proof of Theorem~\ref{thm:elimination} can be found in the appendix.\todo{add proof}

Hence, without loss of generality, we can restrict our Hoare logic proofs for object-oriented programs
to have no adaption rule applications interspersed with the structural rules listed in
Theorem~\ref{thm:reordering} and at most one application of the CONS rule before any axiom application.

Next, we need to show the equivalence of the proof systems for \textbf{dyn} programs and those for object-oriented
programs given in \cite{AptDeBoerOlderog2012}.
We thus wish to show that a correctness formula $\{p\} S \{q\}$ is derivable in the proof system for dyn
iff its translation $\{\Theta(p)\} \Theta(S) \{\Theta(q)\}$ is derivable in the corresponding proof system
for object-oriented programs.

This is stated by Theorem~\ref{thm:translation2} at the end of this section. It will be shown
by induction on the length of the derivation. Before, we have to establish the necessary prerequisites
for the induction step.

We will thus consider each (structural) rule by itself, assuming the inductions hypothesis holds.

\noindent RULE ASGN:
\begin{center}
\def\defaultHypSeparation{\hskip.8pt}
\AxiomC{$\{ p' \} \Theta(E) \{ \Theta(q[v := \result]) \}$}
\LeftLabel{\scriptsize (CONS)}
\UnaryInfC{$\{ p' \} \Theta(E) \{ q'[v := r] \}$}
\AxiomC{\scriptsize (ASGN)}
\doubleLine
\UnaryInfC{$\{ q'[v := r] \} v := r \{ q' \}$}
\LeftLabel{\scriptsize (SEQ)}
\BinaryInfC{$\{ p' \} \Theta(E); v := r \{ q' \}$}
\DisplayProof
\end{center}
where $p' \equiv \Theta(p), q' \equiv \Theta(q), v \in \Var$, using Lemma~\ref{lem:dist_subst_theta}.

For every dyn-derivation applying the ASGN rule, we can construct an object-oriented derivation using
this equivalent sequence of rule applications.
Conversely, every object-oriented proof for a translated
assignment $\Theta(v := E)$ will contain an application of the SEQ rule with a premise of the form
$\{ p' \} \Theta(E) \{ \dot{r} \}$. Note that there could be an application of the CONS rule before the
application of the ASGN axiom (hence the double line). However, since implication and substitution commute
\todo{is this the right terminology?}, we can merge the two implications (pre- and postcondition) into one
on the precondition and state $\dot{r} \rightarrow q'[v := r]$.
Any derivation for the premise $\{ p' \} \Theta(E) \{ \dot{r} \}$ can thus be turned into one for
$\{ p' \} \Theta(E) \{ \Theta(q[v := \result]) \}$ by appending an application of the CONS rule.
The desired biimplication follows immediately.

\noindent RULE COND:
\begin{center}
\AxiomC{$\begin{matrix}
             \{ p' \} \Theta(B) \{ \Theta(\dot{r}) \wedge \mathit{bt} \} & (1) \\ 
             \{ \Theta(\dot{r}) \wedge \mathit{bt} \} S' \{ \Theta(\dot{r}) \wedge \mathit{bt'} \} & (2) \\
             \{ \Theta(\dot{r}) \wedge \mathit{bt'} \} S \{ q' \} & (3) \\
            \end{matrix}$}
\LeftLabel{\scriptsize 2x(SEQ)}
\UnaryInfC{$\{ p' \} \Theta(B); S'; S \{ q' \}$}
\DisplayProof
\end{center}

where $p' \equiv \Theta(p), q' \equiv \Theta(q), v \in \Var$,\newline
$S' \equiv$ if $r \not= \Vnull \rightarrow$ if$_\tau$ $r.@\mathbf{c} = \oC_{\mathit{bool}} \rightarrow r.\mathit{to\_ref}()$ fi fi,\newline
$S \equiv$ if $r \not= \Vnull$ then $\Theta(S_1)$ else $\Theta(S_2)$ fi,
$\mathit{bt} \equiv bool(r,\Theta(b))$

(1) is a direct translation of a premise, (2) can be shown as follows

\begin{center}
\AxiomC{\scriptsize SPEC of $\mathit{to\_ref()}$}
\UnaryInfC{$\begin{matrix}
           \{ \dot{p} \} r.\mathit{to\_ref}() \{ \dot{q} \} \\
           \dot{p} \rightarrow r.@\mathbf{c} = \oC_{\mathit{bool}}
         \end{matrix}$}
\LeftLabel{\scriptsize (FAIL$_\tau$)}
\UnaryInfC{$\begin{matrix}
           \{ \dot{p} \}$ if$_\tau$ $r.@\mathbf{c} = \oC_{\mathit{bool}} \rightarrow r.\mathit{to\_ref}()$ fi $\{ \dot{q} \} \\
           \dot{p} \rightarrow r \not= \Vnull
         \end{matrix}$}
\LeftLabel{\scriptsize (FAIL)}
\UnaryInfC{$\{ \dot{p} \} S' \{ \dot{q} \}$}
\DisplayProof
\end{center}
where $\dot{p} \equiv \Theta(\dot{r}) \wedge \mathit{bt}, \dot{q} \equiv \Theta(\dot{r}) \wedge \mathit{bt'}, \mathit{bt'} \equiv \Theta(b) \leftrightarrow r \not= \Vnull$
using $\{\mathit{bool}(o,\dot{b}) \wedge p\} o.\mathit{to\_ref}() \{r \not= \Vnull \leftrightarrow \dot{b} \wedge p\}$ as SPEC of $\mathit{to\_ref()}$.

(3) can be reduced to translations of the 2 other premises

\begin{center}
\AxiomC{$\begin{matrix}
           \{ \Theta(\dot{r}) \wedge \Theta(b) \} \Theta(S_1) \{ q' \} \\
           \{ \Theta(\dot{r}) \wedge  \neg \Theta(b) \} \Theta(S_2) \{ q' \}
         \end{matrix}$}
\LeftLabel{\scriptsize 2x(CONS)}
\UnaryInfC{$\begin{matrix}
           \{ \Theta(\dot{r}) \wedge \mathit{bt'} \wedge r \not= \Vnull \} \Theta(S_1) \{ q' \} \\
           \{ \Theta(\dot{r}) \wedge \mathit{bt'} \wedge r = \Vnull \} \Theta(S_2) \{ q' \}
         \end{matrix}$}
\LeftLabel{\scriptsize (COND)}
\UnaryInfC{$\{ \Theta(\dot{r}) \wedge \mathit{bt'} \} S \{ q' \}$}
\DisplayProof
\end{center}
\todo{other notions of correctness}

\todo{LOOP rule}

\noindent RULE METH:
\begin{center}
\AxiomC{$\begin{matrix}
             \{  \Theta(p_i) \} S_i \{ \Theta(p_{i+1}) \} \text{ for all }i \in \mathbb{N}_n & (1) \\ 
             \{ \Theta(p_{n+1}) \} S \{ \Theta(q) \} & (2)
            \end{matrix}$}
\LeftLabel{\scriptsize $(n+1)$x(SEQ)}
\UnaryInfC{$\{ \Theta(p_0) \} S_0;...;S_n;S \{ \Theta(q) \}$}
\DisplayProof
\end{center}
%
where $S_i \equiv \Theta(E_i);l_i := r$ for all $i \in \mathbb{N}_n$, $S \equiv \Theta(l_0.m(l_1,...,l_n))$.

(2) is a translated premise and all $n+1$ instances of (1) can be reduced to one as follows

\begin{center}
\AxiomC{$\{ p' \} \Theta(E_i) \{ \Theta(p_{i+1}[l_i := \result]) \}$}
\RightLabel{\scriptsize I}
\UnaryInfC{$\{ p' \} \Theta(E_i) \{ \dot{p} \}$}
\AxiomC{\scriptsize (ASGN)}
\UnaryInfC{$\{ \dot{p} \} l_i := r \{ \Theta(p_{i+1}) \}$}
\LeftLabel{\scriptsize (SEQ)}
\BinaryInfC{$\{ p' \} \Theta(E_i); l_i := r \{ \Theta(p_{i+1}) \}$}
\DisplayProof
\end{center}
%
where $p' \equiv \Theta(p_i), \dot{p} \equiv \Theta(p_{i+1})[l_i := r]$ and I marks an
application of the CONS rule using Lemma~\ref{lem:dist_subst_theta}.

\vspace{0.1cm}
\noindent RULE REC:
In a translated \textbf{dyn} program, all methods (originally having arity $n$) are named $m@C$ and
take $\Var_L \setminus \Var_S$ arguments, where
all arguments following the first $n$ are set to $\Vnull$ on every method call. The set of method call
assumptions thus has the form
%
\begin{align*}
A' \equiv \{ \{ \Theta(p_1) \} s_1.m_1@C_1(\Vector{l_1},\Vector{\Vnull}) \{ \Theta(q_1) \}, ...,\\
\{ \Theta(p_n) \} s_n.m_n@C_n(\Vector{l_n},\Vector{\Vnull}) \{ \Theta(q_n) \} \}
\end{align*}
%
First, we establish the following lemma
%
\begin{lemma} \textbf{Method call}\newline
\label{lem:method_call}
For all sets of assumptions about method calls $A$ and all
assertions $\Theta(p)$ with $\Theta(p) \rightarrow s \not= \Vnull \wedge s.@\mathbf{c} = \oC_{C}$,
\[ A \vdash \{ \Theta(p) \} \Theta(s.m(\Vector{l})) \{ \Theta(q) \} \]
iff
\[ A \vdash \{ \Theta(p) \} s.m@C(\Vector{l},\Vector{\Vnull}) \{ \Theta(q) \} \]
\end{lemma}
%
\textbf{Proof.}
\begin{center}
\AxiomC{$\{ p' \}$ $S_k$ $\{ q' \}$}
\AxiomC{$p' \rightarrow s \not= \Vnull$}
\RightLabel{\scriptsize (FAIL)}
\BinaryInfC{$\{ p' \}$ if $s \not= \Vnull \rightarrow S_k$ fi $\{ q' \}$}
\RightLabel{\scriptsize $\equiv$}
\UnaryInfC{$\{ p' \} \Theta(s.m(\Vector{l})) \{ q' \}$}
\DisplayProof
\end{center}
where $p' \equiv \Theta(p), q' \equiv \Theta(q)$.

Note that every derivation for $\{ p' \} \Theta(s.m(\Vector{l})) \{ q' \}$ neccessarily contains
an application of the FAIL rule and thus a derivation for it's premise $\{ p' \}$ $S_k$ $\{ q' \}$.
When $p' \rightarrow s \not= \Vnull$ holds, we can thus state the biimplication
%
\begin{equation}
\label{eq:biimp_first_step}
 A \vdash \{ p' \} \Theta(s.m(\Vector{l})) \{ q' \} \text{\hspace{0.5cm} iff \hspace{0.5cm}} A \vdash \{ p' \} S_k \{ q' \}
\end{equation}
%
The latter can be shown by induction over the structure of $S_k$.

\noindent Base case: $\{ false \}$ if$_\tau$ $\mathit{false} \rightarrow \mathit{skip}$ fi $\{ q' \}$ \newline
Induction step: We assume that $\{C'_1,...,C'_k\}$ is the set of all
classes supporting the method $m$ of the right arity, then for all $j \in \mathbb{N}^1_k$

\begin{center}
\AxiomC{$\{ p' \} M_j \{ q' \}$}
\RightLabel{$\ll$}
\UnaryInfC{$\{ p' \wedge \dot{c}_j \wedge c_j \} M_j \{ q' \}$}
\AxiomC{$\{ p' \wedge \dot{c}_{j-1} \} S_{j-1} \{ q' \}$}
\RightLabel{\scriptsize (COND)}
\BinaryInfC{$\{ p' \wedge \dot{c}_j \}$ if $c_j$ then $M_j$ else $S_{j-1}$ fi $\{ q' \}$}
\RightLabel{\scriptsize $\equiv$}
\UnaryInfC{$\{ p' \wedge \dot{c}_j \} S_j \{ q' \}$}
\DisplayProof
\end{center}
where $c_j \equiv s.@\mathbf{c} = \oC_{C'_j}$, $\dot{c}_j \equiv \bigwedge^k_{i = j+1} \neg c_i$,
$M_j \equiv s.m@C_j(\Vector{l},\Vector{\Vnull})$.

Since $p' \rightarrow s.@\mathbf{c} = \oC_C$ and assuming that $C$ supports the method $m$ of the
right arity, there is exactly one $j \in \mathbb{N}^1_k$, for which $p' \wedge c_j$ holds
($C'_j = C$). Since $\{ false \} M_j \{ q' \}$ is trivial to establish, this case is the only
one remaining from all premises on the left. As the precondition $p' \wedge \dot{c}_0$
is unsatisfiable, the base case takes care of the fall-though case $S_0$. Thus
the only remaining premise is $\{ p' \} M_j \{ q' \}$ for the case $C'_j = C$.

Note that every derivation for $\{ p' \} S_k \{ q' \}$ ($\dot{c}_k \equiv \mathit{true}$) neccessarily
contains $k$ applications of the COND rule and (assuming that $C$ supports the method $m$ of the
right arity) a derivation for the one premise $\{ p' \wedge \dot{c}_j \wedge c_j \} M_j \{ q' \}$ with
a satisfiable precondition. Since in this case $C'_j = C$, it holds that $p' \rightarrow c_j \wedge \dot{c}_j$.
Thus $p' \wedge c_j \wedge \dot{c}_j \leftrightarrow p'$ and the application of the CONS rule marked with
$\ll$ is also a biimplication. It follows that
%
\begin{equation*}
 A \vdash \{ p' \} S_k \{ q' \} \text{\hspace{0.5cm} iff \hspace{0.5cm}} A \vdash  \{ p' \} M_j \{ q' \}
\end{equation*}
%
Combined with (\ref{eq:biimp_first_step}), the desired result follows. $\Box$
\vspace{0.1cm}

Now the derivation for the REC rule is as follows
%
\begin{center}
\AxiomC{$\begin{matrix}
             \Theta(A) \vdash \{ \Theta(p) \} \Theta(S) \{ \Theta(q) \} & (1') \\ 
             \hspace*{-1cm}\Theta(A) \vdash \{ \Theta(p_i) \} \text{ begin local } \this, \Vector{u_i}, \Vector{h_i} := \\
             s_i, \Vector{l_i}, \Vector{\Vnull}; \Theta(S_i) \text{ end } \{ \Theta(q_i) \}, i \in \mathbb{N}^1_n & (2') \\
             \Theta(p_i) \rightarrow s_i \not= \Vnull \wedge s_i.@\mathbf{c} = \oC_{C_i} \text{ for } i \in \mathbb{N}^1_n & (3')
            \end{matrix}$}
\LeftLabel{\scriptsize $\gg$}
\UnaryInfC{$\begin{matrix}
             A' \vdash \{ \Theta(p) \} \Theta(S) \{ \Theta(q) \} & (1) \\ 
             \hspace*{-1cm}A' \vdash \{ \Theta(p_i) \} \text{ begin local } \this, \Vector{u_i}, \Vector{h_i} := \\
             s_i, \Vector{l_i}, \Vector{\Vnull}; \Theta(S_i) \text{ end } \{ \Theta(q_i) \}, i \in \mathbb{N}^1_n & (2) \\
             \Theta(p_i) \rightarrow s_i \not= \Vnull, i \in \mathbb{N}^1_n & (3)
            \end{matrix}$}
\LeftLabel{\scriptsize (REC)}
\UnaryInfC{$\{ \Theta(p) \} \Theta(S) \{ \Theta(q) \}$}
\DisplayProof
\end{center}
%
where
\begin{align*}
 \Theta(A) \equiv \{ \{ \Theta(p_1) \} \Theta(s_1.m_1(\Vector{l_1})) \{ \Theta(q_1) \}, ..., \\
 \{ \Theta(p_n) \} \Theta(s_n.m_n(\Vector{l_n})) \{ \Theta(q_n) \} \}
\end{align*}

$\gg$ marks an implication strengthening the premises. For all $i \in \mathbb{N}^1_n$ and
under the assumption $(3')$,
$A' \vdash \{ \Theta(p_i) \} \Theta(s_i.m_i(\Vector{l_i})) \{ \Theta(q_i) \}$ 
according to
Lemma~\ref{lem:method_call}. Hence, we state that $A' \vdash \Theta(A)$. It follows that $\Theta(A) \vdash P$
implies $A' \vdash P$ for all statements $P$ and thus $(1') \rightarrow (1)$ and $(2') \rightarrow (2)$.
$(3') \rightarrow (3)$ is also easy to see. $(1')$, $(2')$ and $(3')$ are the translated premises of the REC rule.

\noindent RULE NEW:
\begin{center}
\AxiomC{\scriptsize (NEW)}
\UnaryInfC{$\{ \ddot{p} \} r := \mathbf{new} \{ \dot{p} \}$}
\AxiomC{\scriptsize (ASGN)}
\UnaryInfC{$\{ \dot{p} \} r.@\mathbf{c} := \oC_C \{ \Theta(p) \}$}
\LeftLabel{\scriptsize (SEQ)}
\BinaryInfC{$\{ \ddot{p} \} S \{ \Theta(p) \}$}
\LeftLabel{\scriptsize (CONS)}
\UnaryInfC{$\{ \Theta(p[\result := \mathbf{new}_C]) \} S \{ \Theta(p) \}$}
\DisplayProof
\end{center}
where $\dot{p} \equiv \Theta(q)[r.@\mathbf{c} := \oC_C], \ddot{p} \equiv \dot{p}[r := \mathbf{new}]$,
$S \equiv r := \mathbf{new}; r.@\mathbf{c} := \oC_C$ using Lemma~\ref{lem:dist_new_theta}.


\begin{theorem} \textbf{Translation II}
 \label{thm:translation2}
 For all correctness formulas $\{p\} S \{q\}$, where $S$ is a dyn-program
\begin{equation*}
 \vdash \{p\} S \{q\} \text{\hspace{0.5cm} iff \hspace{0.5cm}} \vdash \{\Theta(p)\} \Theta(S) \{\Theta(q)\}
\end{equation*}
 where $\vdash$ on the left denotes derivability in the proof system for 
 strong typesafe partial correctness of \textbf{dyn} programs and $\vdash$ on the right denotes
 derivability in the proof system for strong partial correctness of object-oriented programs. 
\todo{other notions of correctness}
\end{theorem}

\begin{proof}
 \todo{write}
\end{proof}

\subsection{Completeness}

From the above theorem it immediately follows that the proof system $X$ is sound and (relative) complete
if and only if the proof system $\mathrm{SPO}^+$ for object oriented programs with object creation is.

\subsection{Completeness of Object Oriented Programs with Object Creation}

In \cite{AptDeBoerOlderog2012}, completeness of the two proof systems $\mathrm{SPO}$ and $\mathrm{SPO}^+$ 
for strong partial correctness of object oriented programs is shown. Unfortunately, these proof systems
do not include object creation. We thus extend them by the following rules from \cite{AptDeBoerOlderogBook2009}:

\vspace{0.1cm}

\noindent AXIOM OBJECT CREATION:
\[ \{p[x := \mathbf{new}]\} x := \mathbf{new} \{p\} \]
where $x \in \VarOO$ is a simple object variable and $p$ is a pure assertion.

\vspace{0.1cm}

\noindent RULE OBJECT CREATION:
\begin{center}
\AxiomC{$p' \rightarrow p[u := x]$}
\UnaryInfC{$\{ p'[x := \mathbf{new}] \} u := \mathbf{new} \{ p \}$}
\DisplayProof
\end{center}
where $u$ is a subscripted normal object variable or a (possibly subscripted) instance object variable,
$x \in \VarOO$ is a fresh simple object variable which does not occur in $p$, and $p'$ is a pure assertion.

While the soundness of these rules is shown in \cite{AptDeBoerOlderog2012}, completeness is omitted. We
thus account for it in this paper.


\begin{lemma} \textbf{Completeness: Most General Correctness Formulas for Object Creation}
\label{lem:comp_of_object_creation}
 Let $\Vector{x} = x_1,...,x_k$ be all the variables (global and local) appearing in $D,S,p$ or $q$
 and $\Vector{y}$ be a corresponding sequence of fresh variables. Further, let $q$ be a consistent
 assertion, i.e. there exists a proper state $\sigma$ for which $\sigma \models q$.
 We fix $S \equiv u := \mathbf{new}$. Then for some $j \in \mathbb{N}^1_k$, $x_j \equiv u$. We denote
 by $\Vector{x'} = x_1,...,x_{j-1},x_{j+1},...,x_k$ and by $\Vector{y'}$ the corresponding subsequence
 of $\Vector{y}$. Also, $u.\Vector{x} = u.x_1,...,u.x_h$ denotes the sequence of all instance variables
 of $u$ and $\Vector{y_u}$ a corresponding sequence of fresh variables.
 We then have
 \[ \models_{sp} \{p\} S \{q\} \text{ implies } \{ WP_{sp}(S,\mathrm{MGP}) \} S \{ \mathrm{MGP} \} \vdash \{p\} S \{q\} \]
 where
 \[ \mathrm{MGP} \equiv \Vector{x'} = \Vector{y'} \wedge u.\Vector{x} = \Vector{y_u} \]
\end{lemma}

\newcommand{\Sub}{[\mathit{Sub}]}
\newcommand{\MGP}{\mathrm{MGP}}
\newcommand{\MGS}{\mathrm{MGS}}
\begin{proof}
 Let $\models_{sp} \{p\} S \{q\}$ with $q$ a consistent assertion. Without loss of generality we may
 assume that $p$ and $q$ do not refer to the variables $\Vector{y}$ or $\Vector{y_u}$ (otherwise,
 we rename them and apply the substitution rule). Applying the invariance rule we obtain
 \[ \{ \MGS(q) \wedge WP_{sp}(S,\MGP) \} S \{ \MGS(q) \wedge \MGP \} \]
 where
 \[ \MGS(q) \equiv q[u.\Vector{x} := \Vector{y_u}][\Vector{x'} := \Vector{y'}][(u = u) := \mathit{true}][(u = t) := \mathit{false}] \]
 here, the substitution $[(u = t) := \mathit{false}]$ is meant to replace every subexpression of the form
 $u = t$ (where $t \not\equiv u$) by the boolean expression $\mathit{false}$. This includes terms of the form
 $t = u$. Note that as required by the invariance rule, $\MGS(q)$ does not refer to any variable in
 $\Vector{x}$ (including $u$), even though $q$ can.
 
 The postcondition implies $q$, as the information contained in $\MGP$ allows resubstitution of
 the variables and substituting $u = u$ for $\mathit{true}$ and $u = t$ for some $t \not\equiv u$ for
 $\mathit{false}$ does not change the truth of an assertion due to the uniqueness of the newly created objects
 referred to by $u$. By the consequence rule, we thus obtain
 \[ \{ \MGS(q) \wedge WP_{sp}(S,\MGP) \} S \{ q \} \]
 Next we apply the auxiliary rule for introduction of existential quantification:
 \[ \{ \exists \Vector{y'},\Vector{y_u} \bullet \mathrm{MGS}(q) \wedge WP_{sp}(S,\mathrm{MGP}) \} S \{ q \} \]
 
 By definition of the weakest precondition and $\models_{sp} \{p\} S \{q\}$, it follows that $p$ implies
 the above precondition (an application of the consequence rule thus gives us the desired correctness
 formula): Let $\sigma \models p$. It follows from $\models_{sp} \{p\} S \{q\}$ that
 $\mathcal{M}_{sp}\llbracket S \rrbracket(\sigma) \subseteq \llbracket q \rrbracket$, i.e.
 $\mathcal{M}_{sp}\llbracket S \rrbracket(\sigma) = \emptyset$ or $\sigma' \in \mathcal{M}_{sp}\llbracket S \rrbracket(\sigma)$,
 for some proper state $\sigma'$.
 
 The first case cannot occur as $u := \mathbf{new}$ always terminates.
 
 We thus consider the case that $\sigma' \in \mathcal{M}_{sp}\llbracket S \rrbracket(\sigma)$, for some proper state
 $\sigma'$. From the Semantic Invariance Lemma \cite[Lemma 8.1]{AptDeBoerOlderog2012} it follows that
 $\sigma' \in \mathcal{M}_{sp}\llbracket S \rrbracket(\sigma)$ implies $\sigma'\Sub \in \mathcal{M}_{sp}\llbracket S \rrbracket(\sigma\Sub)$
 with $\Sub \equiv [\Vector{y'} := \sigma'(\Vector{x'})][\Vector{y_u} := \sigma'(u.\Vector{x})]$.
 Clearly, $\sigma'\Sub \models \MGP$, and therefore $\sigma\Sub \models WP_{sp}(S,\MGP)$.
 Further, since $\Vector{y}$ are assumed not to appear in $p$, $\sigma \models p$ implies $\sigma\Sub \models p$.
 So we derive from the assumption $\models_{sp} \{p\} S \{q\}$ that $\sigma'\Sub \models q$.
 By the Substitution Lemma \cite[Lemma 9.1]{AptDeBoerOlderog2012}, the fact that $u = u$ is a tautology and
 the uniqueness of the newly created object referred to by $u$, it then follows that
 $\sigma'\Sub \models \MGS(q)$.
 Since $\sigma$ and $\sigma'$ are equal on all variables except those in $\Vector{x}$ and the evaluation
 of $\MGS(q)$ does not depend on the interpretation of the variables $\Vector{x}$, we have also
 $\sigma\Sub \models \MGS(q)$. Summarizing, we obtain that
 \[ \sigma\Sub \models \MGS(q) \wedge WP_{sp}(S,\MGP) \]
 that is,
 \[ \sigma \models \exists \Vector{y'},\Vector{y_u} \bullet \MGS(q) \wedge WP_{sp}(S,\MGP). \]
 \flushright{$\Box$}
 
 \todo{introduct missing notation}
 \todo{is this sufficient to show completeness for OO-programs with object creation?}
 
\end{proof}


\fi


% \subsection{Completeness}
% \label{sec:completeness}
% 
% The relative completeness proof for the given Hoare logic is an important future work. It is not essential,
% as the concepts presented in this paper can be applied to any Hoare logic for dynamically typed
% programs
% and it is reasonable to assume that there is a sound and relative complete one just like there is for
% object-oriented programs \cite{AptDeBoerOlderog2012}.
% The proof would however strengthen the approach as it would show that all typesafe programs can
% indeed be proven typesafe (modulo implication).





==> sections/proofs_are_typings.tex <==

% 
% 
% \todo{define most precise typing}
% 
% 
% 
% \todo{necessary?}
% While translating a precise typing into a kind that does not support its precision is not overly useful,
% the reverse direction makes sense especially for typings that are inconsistent (contain type errors).
% In this case, the translation allows coupling two type inference algorithms of differing precision (and
% usually also differing runtime). The fast, imprecise algorithm $A$ quickly derives a typing $s$ that is safe,
% but often contains a few cases $S_1,...,S_n$ where it is too imprecise to establish type safety
% ($s(S_i) \not\sqsubseteq \smin_P(S_i)$ for $i \in \mathbb{N}^1_n$). Now translating $s$ to $s'$ which is
% of the kind of a more powerful algorithm $A'$ allows applying $A'$
% in a focused way to refine those program locations whose typing is inconsistent with the methods only
% available in $A'$.
% 
% %\subsection{Proofs are Typings}
% 
% In an effort to increase the precision, one can imagine an algorithm that
% from a given set of start states $\Upsilon$, simulating all possible executions of the program $P$
% and for all expressions $S \in dom(\smin_P)$ tracks what values they are evaluated to and calculates
% a minimal type $t_S = \bigsqcup t_i$ where $t_i$ are the types of these values. We call the
% typing this algorithm produces the \emph{most precise typing} and use it as a benchmark for precision.
% In fact, a program $P$ is typesafe iff its most precise typing is consistent. It should be clear,
% however, that the algorithm is computationally infeasible for any but the simplest programs.
% 
% Fortunately, there is an alternative kind of typing that can be used as a target kind for translating
% all other kinds without loosing precision:
% Hoare logic proofs for typesafe partial correctness can also
% be regarded as typings. The minimal type information can be extracted from the type safety preconditions
% in the proof rule applications for method calls, conditionals and while loops. The proof itself is
% stored in the typing as additional information and its safety verified using the rules of Hoare logic
% and the logic used as its respective assertion language. If the Hoare logic used is (relative) complete,
% then -- assuming one is able to proof all implications -- such a proof exists for all typesafe programs,
% making the precision of Hoare logic typings equivalent to most precise typings. Unfortunately, like for
% most precise typings, there is a drawback: finding such Hoare logic proofs for a given program is undecidable.
% The proofs must hence be manually constructed. However, not only do modern theorem provers offer a significant
% amount of automation, the typing translation discussed earlier allows turning the most powerful automated
% type safety verifiers available into automated proof generators. Like in the previous section, instead
% of manually deriving the entire type safety proof, one takes a generated one containing a few inconsistencies
% and repairs these manually.
% 

